M\'etodo de Monte Carlo aplicado ao C\'alculo Fracion\'ario

This article analyzes and develops a method to solve fractional ordinary differential equations using the Monte Carlo Method. A numerical simulation is performed for some differential equations, comparing the results with what exists in the mathematical literature. The Python language is used to create computational models.

==> Arquivados/biblio.tex <==
   
     \bibitem[OLDHAM ; SPANIER, 1974]{OldhamSpanier} 
    OLDHAM, K.B., SPANIER, K. B. {\bf The Fractional Calculus}. New York: Academic Press, 1974.
    
    \bibitem[PODLUBNY, 2002]{Podlubny}
    PODLUBNY, I. Geometric and physical interpretation of fractional integration and fractional differentiation. \textit{Frac. Calc. \& Appl. Anal.}, 5, 367-386, 2002.
    
    \bibitem[MAINARDI, 2010]{mainardi} MAINARDI, F. {\bf Fractional Calculus and Waves in Linear Viscoelasticity: An Introduction to Mathematical Models}. Singapore: World Scientific, 2010.
    
    \bibitem[HILFER, 2000]{Hilfer} HILFER, R., {\bf Applications of Fractional Calculus in Physics}. Singapore: World Scientific, 2000.
    
    \bibitem[SABATIER; AGRAWAL; MACHADO, 2007]{SATM} SABATIER, J., AGRAWAL, O. P., TENREIRO MACHADO, J. A. {\bf Advances in Fractional Calculus: Theoretical Developments and Applications in Physics and Engineering}. Netherlands: Springer, 2007.
    
    \bibitem[MAGIN, 2006]{Magin}  MAGIN, R. L. {\bf Fractional Calculus in Bioengineering}.Redding: Begell House, 2006.
   
    \bibitem[DIETHELM, 2004]{KD} DIETHELM, K. {\bf The Analysis of Fractional Differential Equations}. Lectures Notes in Mathematics. London: Springer Verlag, 2004.
    
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
   \bibitem{MC2} AKHTAR, MUHAMMAD NAVEED., DURAD, MUHAMMAD HANIF., AHMED, ASAD. 
    Solving initial value ordinary differential equations by Monte Carlo method. \textit{Proceedings of IAM}, 4, 149-174, 2015.
    
     \bibitem[BAUER, 1958]{MC0}
    BAUER, W. F.  The Monte Carlo Method }.\textit{Journal of the Society for Industrial and Applied Mathematics}, 6(4), 438–451, 1958.
    
    \bibitem[CANTRELL; COSNER, 2003]{robert} CANTRELL, R.S., COSNER, C. {\bf Spartial Ecology via Reaction-Diffusion Equations}. England: Wiley series in mathematical and computational biology, 2003.

    

    
     \bibitem[HULL; DOBELL, 1962]{MC12}
    HULL, T.E., DOBELL, A. R. Random Number Generators, \textit{SIAM Rev}. , 4(3) , 230–254, 1962.
    
    \bibitem [KELLER {\it et al}, 2007]{MC1} KELLER, A., HEINRICH, S., NEIDERREITER, H. {\bf Monte Carlo and Quasi-Monte Carlo Methods 2006}. Berlin: Springer Science \& Business Media, 2007.

    \bibitem[KILBAS; SRIVASTAVA; TRUJILLO, 2006]{kilbas} KILBAS, A. A., SRIVASTANA, H. M., TRUJILLO, J. J. {\bf Theory and Applications of Fractional Differential Equations}. Amsterdam: Elsevier, 2006.
    
    
    
    
    \bibitem[METZLER; KLAFFER, 2000]{random} METZLER, R., KLAFFERK, J. The Random walk's guide to anomalous diffusion: A fracional dynamics approach,
    \textit{Physics Reports}, 339, 1-77, 2000.
    
   
    
    \bibitem[OKUBO; SIMON, 2001]{akira}
    OKUBO, A., SIMON, A. LEVIN.{\bf Diffusion and Ecological Problems: Modern Perspectives}.New York: Springer, 2001.
    
   
    \bibitem[RIVEIRO et al, 2013]{rivero} RIVERO, MARGARITA et al. Fractional dynamics of populations. \textit{ Applied Mathematics and Computation}, 218, 3, 1089-1095, 2011.


    \bibitem[VANDERPLAS, 2016]{P1}
    VANDERPLAS, J. {\bf Python data science handbook: Essential tools for working with data }. "O'Reilly Media,Inc.", 2016. 
